ADELT: Transpilation Between Deep Learning Frameworks

We propose the Adversarial DEep Learning Transpiler (ADELT), a novel approach to source-to-source transpilation between deep learning frameworks. ADELT uniquely decouples code skeleton transpilation and API keyword mapping. For code skeleton transpilation, it uses few-shot prompting on large language models (LLMs), while for API keyword mapping, it uses contextual embeddings from a code-specific BERT. These embeddings are trained in a domain-adversarial setup to generate a keyword translation dictionary. ADELT is trained on an unlabeled web-crawled deep learning corpus, without relying on any hand-crafted rules or parallel data. It outperforms state-of-the-art transpilers, improving pass@1 rate by 17.4 pts and 15.0 pts for PyTorch-Keras and PyTorch-MXNet transpilation pairs respectively. We provide open access to our code at https://github.com/gonglinyuan/adelt.

==> contents/limitations.tex <==
\section{Limitations}\label{sec:limitations}

Our method uses a GitHub corpus from Google BigQuery for pretraining and domain-adversarial training, but this corpus, an outdated snapshot of GitHub, does not have newer code. This limitation restricts our experiments to older DL frameworks, excluding newer ones like JAX. However, an updated version of the unlabeled code corpus could potentially overcome these constraints.

==> contents/tables/results_ablation.tex <==
\begin{footnotesize}
\begin{tabular}{lc@{\hspace{0.75\tabcolsep}}cc@{\hspace{0.75\tabcolsep}}cc@{\hspace{0.75\tabcolsep}}cc@{\hspace{0.75\tabcolsep}}cc@{\hspace{0.75\tabcolsep}}c}
\toprule
                           & \multicolumn{6}{c}{Keyword}                                                 & \multicolumn{4}{c}{Source-to-Source}              \\ \cmidrule(lr){2-7} \cmidrule(lr){8-11}
                           & \multicolumn{2}{c}{P@1} & \multicolumn{2}{c}{P@5} & \multicolumn{2}{c}{MRR} & \multicolumn{2}{c}{BLEU} & \multicolumn{2}{c}{F1} \\ \midrule

% \ours (Small)& \adjustbox{bgcolor=green!9}{83.33} & \adjustbox{bgcolor=green!12}{88.18} & \adjustbox{bgcolor=green!8}{91.67} & \adjustbox{bgcolor=green!15}{\textbf{97.73}} & \adjustbox{bgcolor=green!8}{86.22} & \adjustbox{bgcolor=green!13}{92.98} & \adjustbox{bgcolor=green!14}{94.52} & \adjustbox{bgcolor=green!6}{89.59} & \adjustbox{bgcolor=green!13}{81.61} & \adjustbox{bgcolor=green!9}{75.42} \\
% \ours (Base)& \adjustbox{bgcolor=green!11}{\textbf{85.42}} & \adjustbox{bgcolor=green!15}{\textbf{92.27}} & \adjustbox{bgcolor=green!11}{\textbf{93.75}} & \adjustbox{bgcolor=green!15}{\textbf{97.73}} & \adjustbox{bgcolor=green!9}{\textbf{88.12}} & \adjustbox{bgcolor=green!15}{\textbf{95.18}} & \adjustbox{bgcolor=green!15}{\textbf{94.86}} & \adjustbox{bgcolor=green!7}{\textbf{89.66}} & \adjustbox{bgcolor=green!15}{\textbf{84.72}} & \adjustbox{bgcolor=green!9}{74.51} \\ \midrule 
% \multicolumn{11}{l}{\textit{Domain-adversarial training}} \\
% w/o \pretrained (Small)& \adjustbox{bgcolor=red!11}{52.08} & \adjustbox{bgcolor=red!3}{63.64} & \adjustbox{bgcolor=red!15}{70.00} & \adjustbox{bgcolor=green!2}{85.91} & \adjustbox{bgcolor=red!12}{60.54} & \adjustbox{bgcolor=red!2}{72.84} & \adjustbox{bgcolor=red!11}{78.92} & \adjustbox{bgcolor=red!11}{78.66} & \adjustbox{bgcolor=red!13}{38.83} & \adjustbox{bgcolor=red!9}{45.76} \\
% w/o \pretrained (Base)& \adjustbox{bgcolor=red!15}{45.00} & \adjustbox{bgcolor=red!9}{54.55} & \adjustbox{bgcolor=red!15}{70.42} & \adjustbox{bgcolor=red!5}{79.55} & \adjustbox{bgcolor=red!15}{56.81} & \adjustbox{bgcolor=red!8}{65.99} & \adjustbox{bgcolor=red!10}{79.19} & \adjustbox{bgcolor=red!15}{76.35} & \adjustbox{bgcolor=red!15}{35.33} & \adjustbox{bgcolor=red!12}{40.56} \\
% w/o Adv Loss (Small)& \adjustbox{bgcolor=green!4}{74.58} & \adjustbox{bgcolor=green!10}{85.00} & \adjustbox{bgcolor=green!1}{84.58} & \adjustbox{bgcolor=green!15}{\textbf{97.73}} & \adjustbox{bgcolor=green!3}{80.13} & \adjustbox{bgcolor=green!12}{91.54} & \adjustbox{bgcolor=green!5}{88.80} & \adjustbox{bgcolor=green!5}{88.89} & \adjustbox{bgcolor=green!1}{61.00} & \adjustbox{bgcolor=green!8}{72.92} \\
% w/o Adv Loss (Base)& \adjustbox{bgcolor=green!5}{77.08} & \adjustbox{bgcolor=green!13}{88.64} & \adjustbox{bgcolor=green!7}{90.42} & \adjustbox{bgcolor=green!15}{97.27} & \adjustbox{bgcolor=green!5}{82.60} & \adjustbox{bgcolor=green!13}{92.99} & \adjustbox{bgcolor=green!10}{91.58} & \adjustbox{bgcolor=green!3}{87.16} & \adjustbox{bgcolor=green!4}{67.28} & \adjustbox{bgcolor=green!5}{67.85} \\ \midrule
% \multicolumn{11}{l}{\textit{Measure for dictionary generation}} \\
% Dot product (Small)& \adjustbox{bgcolor=red!2}{65.42} & \adjustbox{bgcolor=red!8}{55.45} & \adjustbox{bgcolor=red!4}{80.00} & \adjustbox{bgcolor=red!5}{79.55} & \adjustbox{bgcolor=red!3}{71.78} & \adjustbox{bgcolor=red!7}{67.23} & \adjustbox{bgcolor=green!2}{86.94} & \adjustbox{bgcolor=red!7}{81.59} & \adjustbox{bgcolor=red!1}{58.83} & \adjustbox{bgcolor=red!1}{58.33} \\
% Dot product (Base)& \adjustbox{bgcolor=green!1}{69.58} & \adjustbox{bgcolor=red!2}{65.91} & \adjustbox{bgcolor=green!2}{85.83} & \adjustbox{bgcolor=green!5}{88.64} & \adjustbox{bgcolor=green!0}{76.12} & \adjustbox{bgcolor=green!0}{76.30} & \adjustbox{bgcolor=green!6}{89.60} & \adjustbox{bgcolor=red!8}{80.78} & \adjustbox{bgcolor=green!2}{62.67} & \adjustbox{bgcolor=red!3}{55.00} \\
% Cosine Sim. (Small)& \adjustbox{bgcolor=green!6}{78.58} & \adjustbox{bgcolor=green!12}{87.64} & \adjustbox{bgcolor=green!5}{88.58} & \adjustbox{bgcolor=green!12}{95.36} & \adjustbox{bgcolor=green!5}{82.54} & \adjustbox{bgcolor=green!12}{91.80} & \adjustbox{bgcolor=green!8}{90.56} & \adjustbox{bgcolor=green!5}{88.49} & \adjustbox{bgcolor=green!6}{69.28} & \adjustbox{bgcolor=green!10}{\textbf{76.14}} \\
% Cosine Sim. (Base)& \adjustbox{bgcolor=green!11}{85.25} & \adjustbox{bgcolor=green!14}{89.91} & \adjustbox{bgcolor=green!7}{90.67} & \adjustbox{bgcolor=green!14}{96.73} & \adjustbox{bgcolor=green!9}{87.46} & \adjustbox{bgcolor=green!14}{93.38} & \adjustbox{bgcolor=green!12}{93.21} & \adjustbox{bgcolor=green!4}{88.17} & \adjustbox{bgcolor=green!13}{80.83} & \adjustbox{bgcolor=green!8}{72.87} \\ \bottomrule

\ours (Small)& \adjustbox{bgcolor=green!9}{82.92} & \adjustbox{bgcolor=green!13}{90.00} & \adjustbox{bgcolor=green!8}{\textbf{91.67}} & \adjustbox{bgcolor=green!15}{\textbf{97.73}} & \adjustbox{bgcolor=green!8}{86.97} & \adjustbox{bgcolor=green!14}{94.04} & \adjustbox{bgcolor=green!13}{93.83} & \adjustbox{bgcolor=green!10}{\textbf{92.13}} & \adjustbox{bgcolor=green!12}{80.67} & \adjustbox{bgcolor=green!12}{80.90} \\
\ours (Base)& \adjustbox{bgcolor=green!11}{\textbf{87.08}} & \adjustbox{bgcolor=green!13}{90.00} & \adjustbox{bgcolor=green!8}{\textbf{91.67}} & \adjustbox{bgcolor=green!15}{\textbf{97.73}} & \adjustbox{bgcolor=green!10}{\textbf{89.67}} & \adjustbox{bgcolor=green!14}{93.96} & \adjustbox{bgcolor=green!15}{\textbf{95.32}} & \adjustbox{bgcolor=green!9}{91.29} & \adjustbox{bgcolor=green!15}{\textbf{85.72}} & \adjustbox{bgcolor=green!13}{\textbf{82.01}} \\ \specialrule{0.5pt}{1pt}{1pt}
\multicolumn{11}{l}{\textit{\footnotesize Domain-adversarial training}} \\
w/o \pretrained (Small)& \adjustbox{bgcolor=red!11}{52.08} & \adjustbox{bgcolor=red!3}{63.64} & \adjustbox{bgcolor=red!15}{70.00} & \adjustbox{bgcolor=green!2}{85.91} & \adjustbox{bgcolor=red!12}{60.54} & \adjustbox{bgcolor=red!3}{72.84} & \adjustbox{bgcolor=red!11}{78.92} & \adjustbox{bgcolor=red!11}{78.66} & \adjustbox{bgcolor=red!13}{38.83} & \adjustbox{bgcolor=red!9}{45.76} \\
w/o \pretrained (Base)& \adjustbox{bgcolor=red!15}{45.00} & \adjustbox{bgcolor=red!9}{54.55} & \adjustbox{bgcolor=red!15}{70.42} & \adjustbox{bgcolor=red!5}{79.55} & \adjustbox{bgcolor=red!15}{56.81} & \adjustbox{bgcolor=red!8}{65.99} & \adjustbox{bgcolor=red!11}{79.19} & \adjustbox{bgcolor=red!15}{76.35} & \adjustbox{bgcolor=red!15}{35.33} & \adjustbox{bgcolor=red!12}{40.56} \\
w/o Adv Loss (Small)& \adjustbox{bgcolor=green!7}{80.42} & \adjustbox{bgcolor=green!12}{88.64} & \adjustbox{bgcolor=green!7}{90.00} & \adjustbox{bgcolor=green!15}{\textbf{97.73}} & \adjustbox{bgcolor=green!7}{85.30} & \adjustbox{bgcolor=green!13}{93.06} & \adjustbox{bgcolor=green!5}{88.89} & \adjustbox{bgcolor=green!7}{90.52} & \adjustbox{bgcolor=green!5}{68.67} & \adjustbox{bgcolor=green!9}{76.32} \\
w/o Adv Loss (Base)& \adjustbox{bgcolor=green!11}{86.25} & \adjustbox{bgcolor=green!13}{90.45} & \adjustbox{bgcolor=green!8}{\textbf{91.67}} & \adjustbox{bgcolor=green!15}{\textbf{97.73}} & \adjustbox{bgcolor=green!10}{89.31} & \adjustbox{bgcolor=green!14}{94.27} & \adjustbox{bgcolor=green!13}{94.31} & \adjustbox{bgcolor=red!1}{85.19} & \adjustbox{bgcolor=green!12}{79.89} & \adjustbox{bgcolor=green!9}{75.07} \\ \specialrule{0.5pt}{1pt}{1pt}
\multicolumn{11}{l}{\textit{\footnotesize Measure for dictionary generation}} \\
Inner Product (Small)& \adjustbox{bgcolor=green!8}{81.25} & \adjustbox{bgcolor=green!7}{79.55} & \adjustbox{bgcolor=green!8}{\textbf{91.67}} & \adjustbox{bgcolor=green!7}{90.00} & \adjustbox{bgcolor=green!8}{86.34} & \adjustbox{bgcolor=green!7}{85.38} & \adjustbox{bgcolor=green!12}{93.24} & \adjustbox{bgcolor=green!4}{88.49} & \adjustbox{bgcolor=green!11}{78.67} & \adjustbox{bgcolor=green!10}{77.08} \\
Inner Product (Base)& \adjustbox{bgcolor=green!10}{85.42} & \adjustbox{bgcolor=green!15}{\textbf{93.18}} & \adjustbox{bgcolor=green!8}{\textbf{91.67}} & \adjustbox{bgcolor=green!15}{\textbf{97.73}} & \adjustbox{bgcolor=green!10}{88.84} & \adjustbox{bgcolor=green!15}{\textbf{95.71}} & \adjustbox{bgcolor=green!14}{94.38} & \adjustbox{bgcolor=green!9}{91.75} & \adjustbox{bgcolor=green!13}{82.17} & \adjustbox{bgcolor=green!12}{81.46} \\ \bottomrule


\end{tabular}
\end{footnotesize}

==> contents/tables/results_main.tex <==
\begin{footnotesize}
\begin{tabular}{lc@{\hspace{0.75\tabcolsep}}cc@{\hspace{0.75\tabcolsep}}cc@{\hspace{0.75\tabcolsep}}cc@{\hspace{0.75\tabcolsep}}cc@{\hspace{0.75\tabcolsep}}cc@{\hspace{0.75\tabcolsep}}cc@{\hspace{0.75\tabcolsep}}c}
\toprule
                           & \multicolumn{6}{c}{PyTorch-Keras}                                                 & \multicolumn{6}{c}{PyTorch-MXNet}              \\ \cmidrule(lr){2-7} \cmidrule(lr){8-13}
                           & \multicolumn{2}{c}{BLEU} & \multicolumn{2}{c}{F1} &
                           \multicolumn{2}{c}{EM} & \multicolumn{2}{c}{BLEU} & \multicolumn{2}{c}{F1} & \multicolumn{2}{c}{EM} \\ \midrule

GPT-3 \citep{gpt3}& \adjustbox{bgcolor=red!13}{62.73} & \adjustbox{bgcolor=red!15}{60.85} &  \adjustbox{bgcolor=red!13}{30.58} & \adjustbox{bgcolor=red!10}{35.62} &
\adjustbox{bgcolor=red!8}{26.00} &
\adjustbox{bgcolor=red!6}{29.20} & \adjustbox{bgcolor=red!13}{62.12} & \adjustbox{bgcolor=red!14}{61.21} & \adjustbox{bgcolor=red!12}{25.84} & \adjustbox{bgcolor=red!9}{32.79} &
\adjustbox{bgcolor=red!9}{23.42} &
\adjustbox{bgcolor=red!8}{25.10} \\
Codex \citep{codex}& \adjustbox{bgcolor=red!10}{66.76} & \adjustbox{bgcolor=red!8}{68.53} & \adjustbox{bgcolor=green!3}{62.96} & \adjustbox{bgcolor=green!7}{70.72} &
\adjustbox{bgcolor=green!6}{56.00} &
\adjustbox{bgcolor=green!8}{60.00} &
\adjustbox{bgcolor=red!10}{65.84} & \adjustbox{bgcolor=red!8}{67.44} & \adjustbox{bgcolor=green!4}{57.42} & \adjustbox{bgcolor=green!9}{68.96} &
\adjustbox{bgcolor=green!5}{53.20} & \adjustbox{bgcolor=green!6}{56.46} \\
% \midrule 
% \textit{Fully unsupervised} & & & & & & & & \\
NMT \citep{transcoder}& \adjustbox{bgcolor=red!15}{61.32} & \adjustbox{bgcolor=red!13}{62.76} & \adjustbox{bgcolor=red!15}{27.54} & \adjustbox{bgcolor=red!15}{26.77} &
\adjustbox{bgcolor=red!15}{10.37} & \adjustbox{bgcolor=red!15}{10.10} & \adjustbox{bgcolor=red!15}{59.60} & \adjustbox{bgcolor=red!13}{62.25} & \adjustbox{bgcolor=red!15}{20.38} & \adjustbox{bgcolor=red!14}{21.67} &
\adjustbox{bgcolor=red!15}{10.46} & \adjustbox{bgcolor=red!15}{10.15} \\
Edit Distance (Cased)& \adjustbox{bgcolor=green!1}{78.81} & \adjustbox{bgcolor=green!0}{78.31} & \adjustbox{bgcolor=red!10}{35.83} & \adjustbox{bgcolor=red!11}{34.38} &
\adjustbox{bgcolor=red!9}{23.34} & \adjustbox{bgcolor=red!10}{20.83} &
\adjustbox{bgcolor=green!2}{79.11} & \adjustbox{bgcolor=green!1}{78.30} & \adjustbox{bgcolor=red!6}{37.65} & \adjustbox{bgcolor=red!7}{35.73} &
\adjustbox{bgcolor=red!9}{22.85} & \adjustbox{bgcolor=red!10}{21.07} \\
Edit Distance (Uncased)& \adjustbox{bgcolor=red!2}{76.29} & \adjustbox{bgcolor=green!0}{78.31} & \adjustbox{bgcolor=red!15}{27.50} & \adjustbox{bgcolor=red!11}{34.38} & \adjustbox{bgcolor=red!12}{16.67} & \adjustbox{bgcolor=red!10}{20.83} & \adjustbox{bgcolor=red!0}{76.40} & \adjustbox{bgcolor=green!2}{78.77} & \adjustbox{bgcolor=red!10}{30.77} & \adjustbox{bgcolor=red!7}{35.97} & \adjustbox{bgcolor=red!11}{18.47} & \adjustbox{bgcolor=red!10}{20.12} \\
ADELT (Small)& \adjustbox{bgcolor=green!14}{93.83} & \adjustbox{bgcolor=green!12}{\textbf{92.13}} & \adjustbox{bgcolor=green!12}{80.67} & \adjustbox{bgcolor=green!13}{80.90} & \adjustbox{bgcolor=green!14}{72.67} & \adjustbox{bgcolor=green!13}{71.67} &
\adjustbox{bgcolor=green!14}{92.39} & \adjustbox{bgcolor=green!11}{\textbf{89.80}} & \adjustbox{bgcolor=green!13}{76.63} & \adjustbox{bgcolor=green!10}{70.59} & \adjustbox{bgcolor=green!11}{66.52} & \adjustbox{bgcolor=green!9}{62.88} \\
ADELT (Base)& \adjustbox{bgcolor=green!15}{\textbf{95.32}} & \adjustbox{bgcolor=green!11}{91.29} & \adjustbox{bgcolor=green!15}{\textbf{85.72}} & \adjustbox{bgcolor=green!13}{\textbf{82.01}} & 
\adjustbox{bgcolor=green!15}{\textbf{75.33}} & \adjustbox{bgcolor=green!14}{\textbf{72.50}} &
\adjustbox{bgcolor=green!15}{\textbf{93.93}} & \adjustbox{bgcolor=green!10}{88.62} & \adjustbox{bgcolor=green!15}{\textbf{80.03}} & \adjustbox{bgcolor=green!11}{\textbf{72.05}} &
\adjustbox{bgcolor=green!13}{\textbf{69.98}} & \adjustbox{bgcolor=green!10}{\textbf{63.67}} \\ \bottomrule

\end{tabular}
\end{footnotesize}
